Ghost Imaging of Dark Particles

We propose a new way to use optical tools from quantum imaging and quantum communication to search for physics beyond the standard model. Spontaneous parametric down conversion (SPDC) is a commonly used source of entangled photons in which pump photons convert to a signal-idler pair. We propose to search for "dark SPDC" (dSPDC) events in which a new dark sector particle replaces the idler. Though it does not interact, the presence of a dark particle can be inferred by the properties of the signal photon. Examples of dark states include axion-like-particles and dark photons. We show that the presence of an optical medium opens the phase space of the down-conversion process, or decay, which would be forbidden in vacuum. Search schemes are proposed which employ optical imaging and/or spectroscopy of the signal photons. The signal rates in our proposal scales with the second power of the feeble coupling to new physics, as opposed to light-shining-through-wall experiments whose signal scales with coupling to the fourth. We analyze the characteristics of optical media needed to enhance dSPDC and estimate the rate. A bench-top demonstration of a high resolution ghost imaging measurement is performed employing a Skipper-CCD to demonstrate its utility in a dSPDC search.

==> macros2018.tex <==
\selectlanguage{spanish}%
\ifdefined\MacrosDosMilDieciocho
\else
\newcommand*{\MacrosDosMilDieciocho}{}

\global\long\def\MODULO#1{\left|\,#1\,\right|}%

\global\long\def\PARENTESIS#1{\left(#1\right)}%

\global\long\def\CORCHETES#1{\left[#1\right]}%

\global\long\def\LLAVES#1{\left\{  #1\right\}  }%

\global\long\def\LKEY#1{\left\{  #1\right.}%

\global\long\def\RKEY#1{\left.#1\right\}  }%

\global\long\def\LCORCHETE#1{\left[#1\right.}%

\global\long\def\RCORCHETE#1{\left.#1\right]}%

\global\long\def\LPARENTESIS#1{\left(#1\right.}%

\global\long\def\RPARENTESIS#1{\left.#1\right)}%

\global\long\def\ANGULITOS#1{\left\langle #1\right\rangle }%

\global\long\def\ESPACIOLARGO{\hspace{10mm}}%

\global\long\def\ESPACIOMEDIO{\hspace{5mm}}%

\global\long\def\DEF{\overset{{\scriptscriptstyle \text{def}}}{=}}%

\global\long\def\LLAVEARRIBA#1#2{\overset{{\scriptstyle #2}}{\overbrace{#1}}}%

\global\long\def\LLAVEABAJO#1#2{\underset{{\scriptstyle #2}}{\underbrace{#1}}}%

\global\long\def\REALES{\mathbb{R}}%

\global\long\def\IMAGINARIOS{\mathbb{I}}%

\global\long\def\NATURALES{\mathbb{N}}%

\global\long\def\ENTEROS{\mathbb{Z}}%

\global\long\def\COMPLEJOS{\mathbb{C}}%

\global\long\def\RACIONALES{\mathbb{Q}}%

\global\long\def\DIFERENCIAL{\,\text{d}}%
 

\global\long\def\PRIME{{\vphantom{A}}^{\prime}}%
 

\global\long\def\HAPPY{\smiley}%

\global\long\def\SAD{\overset{\cdot.\cdot}{\frown}}%

\global\long\def\ORDER#1{\mathcal{O}\PARENTESIS{#1}}%

\global\long\def\DIRACDELTA#1{\delta_{D}\PARENTESIS{#1}}%

\newcommandx\KRONEDELTA[1][usedefault, addprefix=\global, 1=ij]{\delta_{#1}}%
 

\global\long\def\HEAVYSIDETHETA#1{\Theta_{H}\PARENTESIS{#1}}%

\newcommandx\LEVICIVITASYMBOL[1][usedefault, addprefix=\global, 1=ijk]{\varepsilon_{#1}}%

\global\long\def\SINC{\text{sinc }}%

\global\long\def\ATAN{\text{atan}}%

\global\long\def\INDICADORA#1{\mathbf{1}\left\{  #1\right\}  }%

\global\long\def\VECTOR#1{\boldsymbol{#1}}%

\global\long\def\VERSOR#1{\hat{\VECTOR{#1}}}%

\global\long\def\IDENTITY{\mathds{1}}%

\global\long\def\CURL{\VECTOR{\nabla}\times}%

\global\long\def\GRADIENT{\VECTOR{\nabla}}%

\global\long\def\DIVERGENCE{\VECTOR{\nabla}\cdot}%
 

\global\long\def\LAPLACIAN{\nabla^{2}}%
 

\global\long\def\REALPART#1{\text{Re}\left(#1\right)}%

\global\long\def\IMAGPART#1{\text{Im}\left(#1\right)}%

\global\long\def\TIENDEA#1{\underset{{\scriptscriptstyle #1}}{\longrightarrow}}%

\global\long\def\EVALUADOEN#1#2#3{\left\lceil #1\right\rfloor _{#2}^{#3}}%

\global\long\def\TERA#1{\text{ T}\unit{#1}}%
 

\global\long\def\GIGA#1{\text{ G}\unit{#1}}%

\global\long\def\MEGA#1{\text{ M}\unit{#1}}%

\global\long\def\KILO#1{\text{ k}\unit{#1}}%

\global\long\def\UNIT#1{\,\unit{#1}}%

\global\long\def\CENTI#1{\text{ c}\unit{#1}}%

\global\long\def\MILI#1{\text{ m}\unit{#1}}%

\global\long\def\MICRO#1{\text{ }\mu\unit{#1}}%

\global\long\def\NANO#1{\text{ n}\unit{#1}}%

\global\long\def\PICO#1{\text{ p}\unit{#1}}%

\global\long\def\FEMTO#1{\text{ f}\unit{#1}}%

\global\long\def\PORDIEZALA#1{\times10^{#1}}%

\global\long\def\PROBABILIDAD#1{\mathbb{P}\left(#1\right)}%

\global\long\def\COLOR#1#2{{\color{#2}{\,#1\,}}}%

\global\long\def\RED#1{\textcolor{red}{#1}}%

\global\long\def\BLUE#1{\COLOR{#1}{blue!80!white}}%

\global\long\def\GREEN#1{\textcolor{green!70!black}{#1}}%

\global\long\def\GRAY#1{\COLOR{#1}{black!30}}%

\global\long\def\GRAY#1{\COLOR{#1}{blue!35!white}}%

\global\long\def\GUNDERBRACE#1#2{\GRAY{\LLAVEABAJO{\COLOR{#1}{black}}{#2}}}%

\global\long\def\RUNDERBRACE#1#2{\RED{\LLAVEABAJO{\COLOR{#1}{black}}{#2}}}%

\global\long\def\BUNDERBRACE#1#2{\BLUE{\LLAVEABAJO{\COLOR{#1}{black}}{#2}}}%

\global\long\def\GUPBRACE#1#2{\GRAY{\LLAVEARRIBA{\COLOR{#1}{black}}{#2}}}%

\global\long\def\RUPBRACE#1#2{\RED{\LLAVEARRIBA{\COLOR{#1}{black}}{#2}}}%

\global\long\def\BUPBRACE#1#2{\BLUE{\LLAVEARRIBA{\COLOR{#1}{black}}{#2}}}%
 

\global\long\def\REDCANCEL#1{\RED{\cancel{{\normalcolor #1}}}}%

\global\long\def\BLUECANCEL#1{{\color{blue}\cancel{{\normalcolor #1}}}}%

\global\long\def\GREENCANCEL#1{\GREEN{\cancel{{\normalcolor #1}}}}%

\global\long\def\BLUECANCELTO#1#2{\BLUE{\cancelto{#2}{{\normalcolor #1}}}}%

\fi % end if\selectlanguage{english}%


